Pretraining End-to-End Keyword Search with Automatically Discovered Acoustic Units

End-to-end (E2E) keyword search (KWS) has emerged as an alternative and complimentary approach to conventional keyword search which depends on the output of automatic speech recognition (ASR) systems. While E2E methods greatly simplify the KWS pipeline, they generally have worse performance than their ASR-based counterparts, which can benefit from pretraining with untranscribed data. In this work, we propose a method for pretraining E2E KWS systems with untranscribed data, which involves using acoustic unit discovery (AUD) to obtain discrete units for untranscribed data and then learning to locate sequences of such units in the speech. We conduct experiments across languages and AUD systems: we show that finetuning such a model significantly outperforms a model trained from scratch, and the performance improvements are generally correlated with the quality of the AUD system used for pretraining.

==> inputfiles/experiments_setup.tex <==
\subsection{Setup}
\subsubsection{Datasets}
\label{sec:experiments:datasets}
\noindent \textbf{Keyword search}:
We test the performance of the proposed scheme on the Libri-light~\Citeph{} and Turkish Broadcast News (BNTr)~\Citeph{} corpora.
For Libri-light, we use the 10 hour Libri-light training set as the transcribed data and test on the standard Librispeech~\Citeph{} sets (dev-clean, test-clean, dev-other and dev-other).
To match the Libri-light training data size, we use a 10-hour subset of BNTR from the VOA channel for training and select two 10-hour subsets from the remaining BNTR data as dev and test sets.

Since neither dataset has official query lists, we randomly select 1500 queries composed of equal proportions of unigrams, bigrams and trigrams for each of the dev and eval sets.
Table~\ref{tab:text_stats} shows the proportion of out-of-vocabulary (OOV) queries.

For Libri-light pretraining, we use the 360-hour set of Librispeech as untranscribed data.
In the case of BNTr, we use the full 180-hour BNTr training set~\footnote{https://catalog.ldc.upenn.edu/LDC2012S06} for pretraining.

We experiment with three text corpora for unpaired training: Babel FLP text, BNTR---unpaired text from the Broadcast News dataset totalling around 180 hours, and text from Turkish Wikipedia.
The first two allow us to impact of using text from the test domains, while Wikipedia stands as a control corpus.

For each language, we use the limited language pack (LLP) subset which contains about 10-hours of training data per language as the paired training data.
We use the text from the full language packs (FLP) as the unpaired text for each language.
These contain 5-6 times as many sentences as the LLP subset.

Each language has a 10-hour development (dev) set and a 5-hour evaluation (eval) set, with a few thousand queries per set.
Table~\ref{tab:text_stats} gives a summary of the text data for each language including the size of the paired text lexicon, the size of the unpaired text lexicon, and the proportion of evaluation queries which are OOV with respect to each text source.
We note that Turkish and Zulu, both agglutinative languages, have larger vocabulary sizes and higher OOV rates.

In addition to these, we use the LLP data from 19 other languages of the Babel corpus (about 190 hours in total) for multilingual pretraining of the KWS model---which was shown to significantly improve KWS performance for~\cite{yusuf2023end}--in order to measure whether and how well the proposed method can be used to improve a multilingually pretrained KWS baseline.
\begin{table}[t]
    \centering
    \caption{OOV rates for the query lists used for each dev/test set.}
    \label{tab:text_stats}
    \centering
    \begin{tabular}{l cc ccc ccc c|cc ccc ccc ccc}
    \toprule
          Dataset & \multicolumn{2}{c}{LS-clean} & \multicolumn{2}{c}{LS-other} & \multicolumn{2}{c}{BNTr} \\
         & Dev & Test & Dev & Test & Dev & Test \\
         \midrule
         OOV-Rate (\%)& 1.1 & 2.6 & 2.5 & 3.6 & 11.9 & 6.3 \\
         \bottomrule
    \end{tabular}
\end{table}

\noindent \textbf{Acoustic unit discovery}: For the supervised phase of H-SHMM training where we estimate the hyper-subspaces ($\{\Matrix{M}_k\}$, and $\{\Matrix{m}_k\}$ in Section~\ref{sec:methods:hshmm}), we use the models from~\Citeph{} which were trained on data from seven languages: French~\Citeph{}, German~\Citeph{}, Polish~\Citeph{} and Spanish~\Citeph{} from the Globalphone corpus~\Citeph{}, and Amharic~\Citeph{}, Swahili~\Citeph{} and Wolof~\Citeph{} from the Alffa project~\Citeph{}.
A 1500-utterance subset of each language (totalling around 19 hours of speech).

For actual acoustic unit discovery, where we learn the acoustic units ($\{\Matrix{\alpha}^l\}, \{\Matrix{\eta}^{l, u}\}$) for each target language, we use random 3000-utterance subsets from each respective language's untranscribed data, and use the learned HMMs to transcribe the full corpus.

\subsubsection{Acoustic features}
The default acoustic inputs to our models (both AUD and KWS) are 13-dimensional MFCC features.
In addition, we consider features from a pretrained 300 million parameter XLS-R model~\cite{babu22_interspeech}~\footnote{https://dl.fbaipublicfiles.com/fairseq/wav2vec/xlsr2\_300m.pt}.
We use the output of the 15th layer, which were to yield considerably better AUD performance in~\Citeph{}.
Note that, due to computational constraints, we only use the XLS-R model as a feature extractor rather than finetune it.

\subsubsection{Metrics}
\noindent \textbf{Term Weighted Value}: In our experiments, we report the term weighted values (TWV)~\cite{Fiscus2007}, which is a measure of weighted recall and precision averaged across queries.
The TWV of a system on a set of queries, $\mathcal{Q}$, at a threshold, $\zeta$, is defined as:
\begin{align}
    \text{TWV} = 100 \times \bigl(1 - \frac{1}{\mathcal{Q}} \sum_{q \in \mathcal{Q}} (P_{miss}(q, \zeta) + \beta P_{FA}(q, \zeta)) \bigr),
    \label{eqn:twv}
\end{align}
where $P_{miss}(q, \zeta)$ is the probability of misses, $P_{FA}(q, \zeta)$ is the probability of false alarms and $\beta$ is a parameter which controls the relative importance of the two.
Following prior NIST evaluations~\cite{Fiscus2007,kws14Evalplan}, we set $\beta=999.9$.
The threshold $~\zeta$ is tuned on the dev sets.
For the dev sets, we report the maximum term weighted value (MTWV) which is the TWV at the threshold which maximizes it.
For the test sets, we report the actual term weighted value (ATWV) which is computed by using the threshold tuned on the dev-set.
% Interested readers can consult~\Citeph{} for a coverage of term weighted value.
% Note that we report all our TWV in percentages, i.e., we always multiply the TWVs as defined in~\ref{eqn:twv} by $100$, so $100\%$ corresponds to a perfect system with no misses and no false alarms, whereas $0\%$ corresponds to a system with no outputs, and negative TWV (up to $-\beta \times 100 \%$) is possible for systems with a preponderance of false alarms.
We adopt keyword-specific thresholding for across-query score normalization~\cite{miller2007rapid} in order to allow various queries with different score distributions to be compared with a single global threshold.

\noindent \textbf{Normalized Mutual Information}: We also report normalized mutual information (NMI) for the AUD systems in order to see how KWS performance varies with the intrinsic quality of the AUD system used for pretraining.
NMI is computed by normalizing the mutual information between discovered units $\mathcal{U}$ and actual reference phones $\mathcal{P}$:
\begin{align}
    \text{NMI}(\mathcal{P}, \mathcal{U}) = 200 \times \frac{I(\mathcal{P}; \mathcal{U})}{H(\mathcal{P}) + H(\mathcal{U})} \%,
\end{align}
and takes values in $[0, 100]$, with 0 denoting completely uncorrelated units and 100 denoting perfect correlation.

\subsubsection{Model configuration and hyper-parameters}
We base the architecture of our model on~\cite{yusuf2023end}.
The query encoder is a network with a 32-dimensional embedding layer for computing vector representations of each input grapheme, followed by 2 bidirectional gated recurrent unit (GRU) layers with 256 output units per direction per layer, and a 400-dimensional output projection layer whose outputs are summed along the sequence dimension to obtain the vectoral query representation.

The document encoder has 6 bidirectional long short-term memory (BLSTM) layers with 512-dimensional output per direction per layer, followed by a 400-dimensional output layer.
We apply dropout of 0.4 between successive BLSTM layers, and down-sample by a factor of 2 after the fourth BLSTM layer.
This results in document encodings with frame durations of 40ms for XLS-R features and 20ms for MFCC.

The H-SHMM use 3-state HMM-GMMs with 4 Gaussians per HMM state, Dirichlet process with truncation parameter of 1, 100-dimensional unit embedding ($| \Matrix{\eta}^{l, u} |$) and 5-dimensional language embedding ($|\Matrix{\alpha}^l|$).

\subsubsection{Training details}
The neural networks are trained with the Adam optimizer~\Citeph{}.
For pretraining, we use a cosine decay schedule with peak learning rate of $5e-4$ and final learning rate of $1e-7$, and train for 200000 steps, with the first 10000 being linear warmup.
For finetuning (and the baseline with no pretraining), we train with the step-based training from~\Citeph{} which we found to work slightly better.
This starts with a learning rate of 0.002 which is halved whenever the validation loss (computed over 10\% of the training queries) does not improve over 4 epochs through the data, and training is stopped when validation loss does not improve for 10 epochs.
